Search for exclusive Higgs and $Z$ boson decays to $\phi\gamma$ and $\rho\gamma$ with the ATLAS detector

A search for the exclusive decays of the Higgs and $Z$ bosons to a $\phi$ or $\rho$ meson and a photon is performed with a $pp$ collision data sample corresponding to an integrated luminosity of up to 35.6 $fb^{-1}$ collected at $\sqrt{s}=13$ TeV with the ATLAS detector at the CERN Large Hadron Collider. These decays have been suggested as a probe of the Higgs boson couplings to light quarks. No significant excess of events is observed above the background, as expected from the Standard Model. Upper limits at 95$\% $ confidence level were obtained on the branching fractions of the Higgs boson decays to $\phi\gamma$ and $\rho\gamma$ of $5.0\times10^{-4}$ and $10.4\times10^{-4}$, respectively. The corresponding 95$\% $ confidence level upper limits for the $Z$ boson decays are $0.7\times10^{-6}$ and $4.0\times10^{-6}$ for $\phi\gamma$ and $\rho\gamma$, respectively.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document

# Copyright (C) 2002-2023 CERN for the benefit of the ATLAS collaboration
#------------------------------------------------------------------------------
# By default makes ANA-HDBS-2018-52-PAPER.pdf using target run_pdflatex.
# Replace ANA-HDBS-2018-52-PAPER with your main filename or add another target set.
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to remove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_pdflatex instead of run_latexmk to use explicit
# pdflatex/biber commands to compile.

# You can use the target version to check your TeX Live version.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
# TLVERS   = $(shell pdflatex --version | grep -Go 'TeX Live [0-9]*' | grep -Go '[0-9].*')
# TWIKI    = https://twiki.cern.ch/twiki/bin/view/AtlasProtected/PubComLaTeXFAQ

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = HPhiGamma

#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make ANA-HDBS-2018-52-PAPER.pdf with latexmk.
default: run_latexmk
# Use pdflatex/biber instead to compile.
# default: run_pdflatex

.PHONY: run_latexmk
.PHONY: newdocument newdocumenttexmf newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover newdata
.PHONY: version clean cleanpdf help

# Check TeX Live version
# version:
# 	@echo "Checking version"
# 	@echo "TLVERS $(TLVERS), TEXLIVE $(TEXLIVE)"
# 	@if [ $(TLVERS) -lt $(TEXLIVE) ]; then \
# 		echo "Your TeX Live version ($(TLVERS)) is older than $(TEXLIVE). Please consult $(TWIKI)"; \
# 	fi

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf: %.tex *.tex bib/*.bib
%.pdf:  %.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: TEMPLATE=atlas-paper
newpaper: newdocument newfiles newpapermetadata newauxmat

newpapertexmf: TEMPLATE=atlas-paper
newpapertexmf: newdocumenttexmf newfiles newpapermetadata newauxmat

newnote: TEMPLATE=atlas-note
newnote: newdocument newfiles newnotemetadata

newnotetexmf: TEMPLATE=atlas-note
newnotetexmf: newdocumenttexmf newfiles newnotemetadata

newbook: TEMPLATE=atlas-book
newbook: newdocument newfiles newpapermetadata

newbooktexmf: TEMPLATE=atlas-book
newbooktexmf: newdocumenttexmf newfiles newpapermetadata

draftcover:
	cp  template/atlas-draft-cover.tex $(BASENAME)-draft-cover.tex

preprintcover:
	cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

newdata:
	sed s/atlas-document/$(BASENAME)/ template/atlas-hepdata-main.tex >$(BASENAME)-hepdata-main.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

newdocument:
	sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex

newdocumenttexmf:
	sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	sed 's/\\RequirePackage{latex\/atlaslatexpath}/% \\RequirePackage{latex\/atlaslatexpath}/' \
	>$(BASENAME).tex

newpapermetadata:
	cp template/atlas-paper-metadata.tex $(BASENAME)-metadata.tex

newnotemetadata:
	cp template/atlas-note-metadata.tex $(BASENAME)-metadata.tex

newfiles:
	echo "% Put you own bibliography entries in this file" > $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newauxmat:
	cp template/atlas-auxmat.tex $(BASENAME)-auxmat.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

help:
	@echo "To create a new paper/CONF Note/PUB Note draft give the command:"
	@echo "make newpaper [BASENAME=ANA-HDBS-2018-52-PAPER]"
	@echo "To create a new ATLAS note draft give the command:"
	@echo "make newnote [BASENAME=ANA-HDBS-2018-52-PAPER]"
	@echo "To create a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=ANA-HDBS-2018-52-PAPER]"
	@echo ""
	@echo "To compile the paper give the command"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly."
	@echo ""
	@echo "To compile the document using latexmk give the command:"
	@echo "make run_latexmk"
	@echo "You can also adjust the 'default' target."
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newpapertexmf|newnotetexmf|newbooktemf [BASENAME=ANA-HDBS-2018-52-PAPER]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=ANA-HDBS-2018-52-PAPER]"
	@echo "pdflatex ANA-HDBS-2018-52-PAPER-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=ANA-HDBS-2018-52-PAPER]"
	@echo "pdflatex ANA-HDBS-2018-52-PAPER-preprint-cover"
	@echo ""
	@echo "If you need a document for HepData material give the commands:"
	@echo "make newdata [BASENAME=ANA-HDBS-2018-52-PAPER]"
	@echo "pdflatex ANA-HDBS-2018-52-PAPER-hepdata-main"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

clean:
	-rm *.toc *.aux *.lof *.lot *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx *.tdo \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp

cleanpdf:
	-rm $(BASENAME).pdf
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-hepdata-main.pdf

cleanall: clean cleanpdf

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^

